3-Dimensional Sonic Phase-invariant Echo Localization

Parallax and Time-of-Flight (ToF) are often regarded as complementary in robotic vision where various light and weather conditions remain challenges for advanced camera-based 3-Dimensional (3-D) reconstruction. To this end, this paper establishes Parallax among Corresponding Echoes (PaCE) to triangulate acoustic ToF pulses from arbitrary sensor positions in 3-D space for the first time. This is achieved through a novel round-trip reflection model that pinpoints targets at the intersection of ellipsoids, which are spanned by sensor locations and detected arrival times. Inter-channel echo association becomes a crucial prerequisite for target detection and is learned from feature similarity obtained by a stack of Siamese Multi-Layer Perceptrons (MLPs). The PaCE algorithm enables phase-invariant 3-D object localization from only 1 isotropic emitter and at least 3 ToF receivers with relaxed sensor position constraints. Experiments are conducted with airborne ultrasound sensor hardware and back this hypothesis with quantitative results.

==> benchmark_table.tex <==
% Benchmark
\begin{table}[!h]
    \centering
    \caption{Comparison}
    \label{tab:comparison}
    \begin{tabular}{l|l|l|l}
        Method & Freq. [kHz] & Sensors~[\#,$\lambda$] & RMSE [cm] \\
        
        \hline
        2-D HFI (EKF)~\cite{Chung-Wei:21} & $40\pm2$ & 6, $\gg\lambda$ & $0.7\pm0.5$ \\%& - \\ %$7.1\pm4.7$mm
        \hline
        3-D Phase correl.~\cite{Toposens:2022} & $40\pm2$ & 3, $\approx\lambda$ & $1.0\pm2.5$ \\
        %\hline
        %3-D Learned sound & $0.02 - 20$ & 2, $\gg\lambda$ & 2.9 \\%& - \\
        \hline
        3-D SPiEL (proposed) & $176\pm1$ & 3, $\gg\lambda$ & $2.4\pm1.5$ \\%& - \\ %3-D SPiEL (
        %\hline%\hline
    \end{tabular}
%\end{IEEEeqnarraybox}
\end{table}

==> field_experiment.tex <==
%drone experiment discussion
	\subsection{Field Experiment}
	PaCE qualifies for navigation and collision avoidance in scenarios that require \mbox{3-D} orientation. To demonstrate its technological capabilities, the prototype is used as an Unmanned Aerial Vehicle (UAV) tracking system, e.g. for landing guidance. Figure~\ref{fig:drone} shows results $\mathbf{s}^\star$ mapped onto the 2-D image plane for intuitive assessment. It is seen that 3 out of 5 positions are detected correctly whereas a false positive outlier and undetected positions indicate limitations of the prototype at this early research stage. Deviations are due to the UAV being a small reflector and a potential domain gap in the learned correspondence of the Siamese MLP, which was trained on the convex robotic target. % and imprecise camera to prototype alignment. %
	%
	\begin{figure}[h]
		\centering
		\includegraphics[trim=200 0 230 220,clip=true,width=.5\linewidth]{./figs/4th_gimp_composition.eps}
		\caption{\textbf{UAV tracking} showing estimates $\mathbf{s}^\star$ as filled circles projected into $x$ and $z$ image dimensions from 5 frames taken every 200~\si{\milli\second}. The circle size encodes $y^\star$ with larger size being closer and blue rings highlight sensors to verify correct image projection. 
		Lines connect estimates $\mathbf{s}^\star$ consecutively during UAV tracking. Demo videos can be found in the supplementary material. \CH{redo with second sequence}\label{fig:drone}}
	\end{figure}
